XL-MIMO Channel Modeling and Prediction for Wireless Power Transfer

Massive antenna arrays form physically large apertures with a beam-focusing capability, leading to outstanding wireless power transfer (WPT) efficiency paired with low radiation levels outside the focusing region. However, leveraging these features requires accurate knowledge of the multipath propagation channel and overcoming the (Rayleigh) fading channel present in typical application scenarios. For that, reciprocity-based beamforming is an optimal solution that estimates the actual channel gains from pilot transmissions on the uplink. But this solution is unsuitable for passive backscatter nodes that are not capable of sending any pilots in the initial access phase. Using measured channel data from an extremely large-scale MIMO (XL-MIMO) testbed, we compare geometry-based planar wavefront and spherical wavefront beamformers with a reciprocity-based beamformer, to address this initial access problem. We also show that we can predict specular multipath components (SMCs) based only on geometric environment information. We demonstrate that a transmit power of 1W is sufficient to transfer more than 1mW of power to a device located at a distance of 12.3m when using a (40x25) array at 3.8GHz. The geometry-based beamformer exploiting predicted SMCs suffers a loss of only 2dB compared with perfect channel state information.

==> AxiDrawPlots.tex <==
\setlength{\figurewidth}{0.4\linewidth}
\setlength{\figureheight}{0.4\linewidth}
\setlength{\hspaceing}{-1.56cm}
% ---------- POSITION 1 ---------- NO SWITCHING OF GRIDS ----------
\begin{figure*}[bt]	% --------------------------------------------------------------------------------------------------------------------
     \hspace{-3mm}
     \begin{subfigure}[t]{0.29\textwidth}
        \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
         \centering
         % ---------- ---------- ---------- ----------
	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
	                \ExcludeFigures% \input{figures/00_MRT_M0.tex}
        \else
            \input{figures/AxiDraw/PW_pos1_switched0.tex}
        \fi % --- exclude figures if necessary---
        % ---------- ---------- ---------- ----------
        \vspace{-2.1mm}
         \caption{\Gls{pw} \gls{los} \gls{bf}}
         \label{fig:PW_pos1_switched0}
     \end{subfigure}%
     \hspace{-1.03cm}%
     \begin{subfigure}[t]{0.29\textwidth}
        \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
         \centering
         % ---------- ---------- ---------- ----------
	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
            \ExcludeFigures
            %\input{figures/02_EB_MRT_M1.tex}
        \else
            \input{figures/AxiDraw/SW_LoS_pos1_switched0.tex}
        \fi % --- exclude figures if necessary---
        % ---------- ---------- ---------- ----------
        \vspace{-2.1mm}
         \caption{\Gls{sw} \gls{los} \gls{bf}}
         \label{fig:SW_LoS_pos1_switched0}
     \end{subfigure}%
     \hspace{\hspaceing}%
     \begin{subfigure}[t]{0.29\textwidth}
         \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
         \centering
         % ---------- ---------- ---------- ----------
	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
            \ExcludeFigures
        \else
            \input{figures/AxiDraw/SW_SMC_pos1_switched0}
        \fi % --- exclude figures if necessary---
        % ---------- ---------- ---------- ----------
        \vspace{-2.1mm}
         \caption{\gls{sw} \gls{smc} \gls{bf}}
         \label{fig:SW_SMC_pos1_switched0}
     \end{subfigure}%
     \hspace{\hspaceing}%
     \begin{subfigure}[t]{0.29\textwidth}
         \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
         \centering
         % ---------- ---------- ---------- ----------
	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
            \ExcludeFigures
        \else
            \input{figures/AxiDraw/CSI_pos1_switched0}
        \fi % --- exclude figures if necessary---
        % ---------- ---------- ---------- ----------
        \vspace{-2.1mm}
         \caption{Reciprocity-based \gls{bf} (full \gls{csi})}
         \label{fig:CSI_pos1_switched0}
     \end{subfigure}%
     \hspace{-0.65cm}%
     \begin{subfigure}[t]{0.058\textwidth}
        \vspace{-2.2mm} %
         \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
         \centering
         %\vspace{-0.5cm}
         %\includegraphics[width=\textwidth,trim={0 0.5cm 0 0.5cm}]{figures/CB.pdf}
                  \setlength{\plotWidth}{1\textwidth}	% NECCESSARY AGAIN!
         	\input{figures/CB.tex}
     \end{subfigure}
    	\vspace{-2.1mm}\caption{
    	Beamformers applied at $\bm{p}_\mrm{EN}^{(1)}$, $PG$ distribution evaluated and interpolated around  $\bm{p}_\mrm{EN}^{(1)}$.
    	}\label{fig:pos1_domains}
    	\vspace{-3mm}
\end{figure*}	% --------------------------------------------------------------------------------------------------------------------
% ---------- POSITION 1 ---------- NO SWITCHING OF GRIDS ----------


% ---------- POSITION 2 ---------- NO SWITCHING OF GRIDS ----------
\begin{figure*}[bt]	% --------------------------------------------------------------------------------------------------------------------
     \hspace{-3mm}
     \begin{subfigure}[t]{0.29\textwidth}
        \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
         \centering
         % ---------- ---------- ---------- ----------
	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
	                \ExcludeFigures
        \else
            \input{figures/AxiDraw/PW_pos2_switched0.tex}
        \fi % --- exclude figures if necessary---
        % ---------- ---------- ---------- ----------
        \vspace{-2.1mm}
         \caption{\Gls{pw} \gls{los} \gls{bf}}
         \label{fig:PW_pos2_switched0}
     \end{subfigure}%
     \hspace{-1.03cm}%
     \begin{subfigure}[t]{0.29\textwidth}
        \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
         \centering
         % ---------- ---------- ---------- ----------
	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
            \ExcludeFigures
        \else
            \vspace{-0.5mm}
            \input{figures/AxiDraw/SW_LoS_pos2_switched0.tex}
        \fi % --- exclude figures if necessary---
        % ---------- ---------- ---------- ----------
        \vspace{-2.1mm}
         \caption{\Gls{sw} \gls{los} \gls{bf}}
         \label{fig:SW_LoS_pos2_switched0}
     \end{subfigure}%
     \hspace{\hspaceing}%
     \begin{subfigure}[t]{0.29\textwidth}
         \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
         \centering
         % ---------- ---------- ---------- ----------
	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
            \ExcludeFigures
        \else
            \vspace{-0.5mm}
            \input{figures/AxiDraw/SW_SMC_pos2_switched0}
        \fi % --- exclude figures if necessary---
        % ---------- ---------- ---------- ----------
        \vspace{-2.1mm}
         \caption{\gls{sw} \gls{smc} \gls{bf}}
         \label{fig:SW_SMC_pos2_switched0}
     \end{subfigure}%
     \hspace{\hspaceing}%
     \begin{subfigure}[t]{0.29\textwidth}
         \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
         \centering
         % ---------- ---------- ---------- ----------
	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
            \ExcludeFigures
        \else
            \vspace{-0.5mm}
            \input{figures/AxiDraw/CSI_pos2_switched0}
        \fi % --- exclude figures if necessary---
        % ---------- ---------- ---------- ----------
        \vspace{-2.1mm}
         \caption{Reciprocity-based \gls{bf} (full \gls{csi})}
         \label{fig:CSI_pos2_switched0}
     \end{subfigure}%
     \hspace{-0.65cm}%
     \begin{subfigure}[t]{0.058\textwidth}
        \vspace{-2.2mm} %
         \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
         \centering
                  \setlength{\plotWidth}{1\textwidth}	% NECCESSARY AGAIN!
         	\input{figures/CB.tex}
     \end{subfigure}
    	\vspace{-1mm}\caption{
    	Beamformers applied at $\bm{p}_\mrm{EN}^{(2)}$, $PG$ distribution evaluated and interpolated around  $\bm{p}_\mrm{EN}^{(2)}$.
    	}\label{fig:pos2_domains}
    	\vspace{-3mm}
\end{figure*}	% --------------------------------------------------------------------------------------------------------------------
% ---------- POSITION 2 ---------- NO SWITCHING OF GRIDS ----------








% SAVE SPACE IF NECESSARY ---------- ----------
\ifdefined\dontreduceSize  
    ~
\else
    % ---------- POSITION 1 ---------- GRIDS SWITCHED! ----------
    \begin{figure*}[bt]	
         \hspace{-3mm}
         \begin{subfigure}[t]{0.29\textwidth}
            \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
             \centering
             % ---------- ---------- ---------- ----------
    	    \ifdefined\ExcludeFigures
    	                \ExcludeFigures
            \else
                \input{figures/AxiDraw/PW_pos1_switched1.tex}
            \fi % --- exclude figures if necessary---
            % ---------- ---------- ---------- ----------
            \vspace{-2.1mm}
             \caption{\Gls{pw} \gls{los} \gls{bf}}
             \label{fig:PW_pos1_switched1}
         \end{subfigure}%
         \hspace{-1.03cm}%
         \begin{subfigure}[t]{0.29\textwidth}
            \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
             \centering
             % ---------- ---------- ---------- ----------
    	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
                \ExcludeFigures
            \else
                \vspace{-0.5mm}
             \input{figures/AxiDraw/SW_LoS_pos1_switched1.tex}
            \fi % --- exclude figures if necessary---
            % ---------- ---------- ---------- ----------
             \vspace{-2.1mm}
             \caption{\Gls{sw} \gls{los} \gls{bf}}
             \label{fig:SW_LoS_pos1_switched1}
         \end{subfigure}%
         \hspace{\hspaceing}%
         \begin{subfigure}[t]{0.29\textwidth}
             \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
             \centering
             % ---------- ---------- ---------- ----------
    	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
                \ExcludeFigures
            \else
                \vspace{-0.5mm}
                \input{figures/AxiDraw/SW_SMC_pos1_switched1}
            \fi % --- exclude figures if necessary---
            % ---------- ---------- ---------- ----------
             \vspace{-2.1mm}
             \caption{\gls{sw} \gls{smc} \gls{bf}}
             \label{fig:SW_SMC_pos1_switched1}
         \end{subfigure}%
         \hspace{\hspaceing}%
         \begin{subfigure}[t]{0.29\textwidth}
             \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
             \centering
             % ---------- ---------- ---------- ----------
    	    \ifdefined\ExcludeFigures   % --- exclude figures if necessary---
                \ExcludeFigures
            \else
                \vspace{-0.5mm}
                \input{figures/AxiDraw/CSI_pos1_switched1}
            \fi % --- exclude figures if necessary---
            % ---------- ---------- ---------- ----------
            \vspace{-2.1mm}
             \caption{Reciprocity-based \gls{bf} (full \gls{csi})}
             \label{fig:CSI_pos1_switched1}
         \end{subfigure}%
         \hspace{-0.65cm}%
         \begin{subfigure}[t]{0.058\textwidth}
            \vspace{-2.2mm} %
             \vskip 0pt	% THIS IS OF UTTERMOST NECESSITY TO MAKE THE TOP "[t]" PARAMETER WORK!
             \centering
                      \setlength{\plotWidth}{1\textwidth}	% NECCESSARY AGAIN!
             	\input{figures/CB.tex}
         \end{subfigure}
        	\vspace{-1mm}\caption{
        	Beamformers applied at $\bm{p}_\mrm{EN}^{(1)}$, $PG$ distribution evaluated and interpolated around  $\bm{p}_\mrm{EN}^{(2)}$.
        	}\label{fig:pos1_domains_switched}
        	\vspace{-3mm}
    \end{figure*}
    % ---------- POSITION 1 ---------- GRIDS SWITCHED! ----------

\fi
% SAVE SPACE IF NECESSARY ---------- ----------



